Speedup and efficiency of computational parallelization: A unifying approach and asymptotic analysis

In high performance computing environments, we observe an ongoing increase in the available numbers of cores. This development calls for re-emphasizing performance (scalability) analysis and speedup laws as suggested in the literature (e.g., Amdahl's law and Gustafson's law), with a focus on asymptotic performance. Understanding speedup and efficiency issues of algorithmic parallelism is useful for several purposes, including the optimization of system operations, temporal predictions on the execution of a program, and the analysis of asymptotic properties and the determination of speedup bounds. However, the literature is fragmented and shows a large diversity and heterogeneity of speedup models and laws. These phenomena make it challenging to obtain an overview of the models and their relationships, to identify the determinants of performance in a given algorithmic and computational context, and, finally, to determine the applicability of performance models and laws to a particular parallel computing setting. In this work, we provide a generic speedup (and thus also efficiency) model for homogeneous computing environments. Our approach generalizes many prominent models suggested in the literature and allows showing that they can be considered special cases of a unifying approach. The genericity of the unifying speedup model is achieved through parameterization. Considering combinations of parameter ranges, we identify six different asymptotic speedup cases and eight different asymptotic efficiency cases. Jointly applying these speedup and efficiency cases, we derive eleven scalability cases, from which we build a scalability typology. Researchers can draw upon our typology to classify their speedup model and to determine the asymptotic behavior when the number of parallel processing units increases. In addition, our results may be used to address various extensions of our setting.

==> content/backgroundMaterial.tex <==
\section{Preliminaries}

Starting with Amdahl's law as a simple theoretical speedup model, we extend this model by consolidating various extensions suggested in the literature and adding new extensions. The ultimate goal is the proposition and analysis of a general theoretical model which allows considering various algorithmic effects of parallelization, including varying (sequential and parallel) workloads induced through varying problem sizes and the reduction of overall workload through parallelization, which enables super-linear speedup\footnote{Quellen nennen: for a limited range of N superlinear speedup occured; Our understanding of super-linear speedup is algorithmic-based rather than based on technical reasons due to architecture specifics, such as those described in \citep[p. 62]{sanders2019sequential}: textit{There are situations where we can do even better. $S > p$ can happen if parallel execution mobilizes more resources. For example, on the parallel machine, the input might fit into the aggregate cache of all PEs while a single PE needs to access the main memory a lot.}. The model is intended to be broadly applicable to analyze scalability issues, including speedup and efficiency, in many algorithmic parallelization scenarios, including mathematical optimization and data analysis.}.  

Our analysis and observations do not focus on or require to have specific parallelization technologies applied (e.g., SMC model, multi-site model, GPGPU, etc.). However, our models assume that all processing units which process the parallel fraction of the code are of equal processing power (they may differ from the processing unit that processes the sequential part of the code).

The fundamental assumption of our models is an Amdahl-type workload that it can be divided into a fully sequential (non-parallelisable, i.e. not affected by the improvement) part and a fully parallel (infinitely parallelisable, i.e. fully affected by the improvement) part\footnote{Two issues with this \citep[p. 140]{al2020amdahl}: issue 1: The focus of this dispute is the fundamental assumption of Amdahl's law, as described by (1), which says that a workload is assumed to consist of two distinct parts, one of which absolutely cannot be parallelised and the other has full (infinite) parallelisability. First of all, infinite parallelisability is difficult to envisage (hence semantically weak) for a workload of fixed size, which Amdahl's law targets. The fundamental atomic element of workloads is usually agreed to be the single instruction. As a workload of fixed size does not expand into an infinite number of instructions, because of the fixed size assumption, it or any part of it should always have non-infinite parallelisability. Secondly, the idea of trying to approximate different degrees of parallelisability with a weighted sum of non- and full-parallelisability may not be regarded as attractive, and has practical limitations. Issue 2: that the p-fraction f is regarded as difficult to determine for workloads not designed on-purpose to fit specific f values. In the aforementioned reference, alternative models (parallelism/span-and-work laws (\citep[p. 772ff]{cormen2022introduction} and \citep[p. 141ff]{al2020amdahl}) and roofline) are summarized. Also, parallelism and p-fractions have been combined, leading to multiple-fraction models for both homogeneous \citep{cassidy2011beyond} and heterogeneous \citep{yun2018estimation} multi-core environments; for an overview see \citep[p. 143ff]{al2020amdahl}} We also assume that the parallel processing units are equally potential in their computing capabilities, such as in SMCs and GPUs. (this might not be the case in heterogenous environments (cmp. Section \ref{sec:archDepLaws}). We also do not consider any load balancing issues, such as task migration (see references 31-34 in \cite{al2020amdahl} and task preemption. Further, we assume single-level parallelism rather than multi-level parallelism, where nested paralleism occurs when, for example, MPI and OpenMP are jointl yused or several GPUs; for multi-level parallelism see,for example, \citep{tang2012speedup}.

     

\begin{itemize}
\item Notation: work/execution time of a single processing unit (PU): $T_1$; execution time of $N$ PUs: $T_N$; speedup: $S_N=\frac{T_1}{T_N}$; efficiency: $E_N=\frac{S_N}{N}=\frac{T_1}{N\cdot T_N}$

\item Amdahl's model: $T_1= s+p$; $T_N=s+\frac{p}{N}$

\item Model with variable problem size and, thus, variable workload/problem size: $T_1= f(N)\cdot s+g(N)\cdot p$; $T_N= f(N)\cdot s+\frac{g(N)\cdot p}{N}$; $\gamma(N)=\frac{g(N)}{f(N)}=N^{\delta,\delta>0}$ \cite[33f\/f]{schmidt2017parallel}
\begin{itemize}
\item $f,g$ account for situations in which problem size and resulting (sequential and parallel) workload vary; in particular, they do not need increase identical to the increase of $N$; see \cite[32f]{trobec2018introduction} for a discusssion on the relationship between numer of parallel processing units $N$ and problem size    
\item $f(N)=g(N)=1 \rightarrow$ Amdahl's law (fixed workload model)
\item $f(N)=1, g(N)=N \rightarrow$ Gustafson's law (fixed time model)
\item $f(n)=1; g(N)=c_1\cdot N^{\alpha} \rightarrow$ my model with flexible effects of parallelization and no change of overall (parallel) workload; i.e., $c_2=1, \beta=1$; $c_1=c_2=1, \beta=1 \leftarrow$ speedup model of Sun and Ni ($\bar g (m)=m^b$ corresponds to $N^{\alpha}$) (memory bounded model) (Section \ref{sec:ModelFlexibleEffects})

\item with $f(N)=1$ and $g(N)=c_1\cdot N^{\alpha}$ the assumption $\gamma(N)=\frac{g(N)}{f(N)}=N^{\delta,\delta>0}$ is violated iff $c_1\neq 1$ or $\alpha \leq 0$
\end{itemize}

\item Model with variable workload and effect of parallelization on overall (parallel) workload (e.g., in b\&b algorithms): $T_1= f(N)\cdot s+g(N)\cdot p$; $T_N= f(N)\cdot s+\frac{g(N)\cdot p}{h(N)}$  
\begin{itemize}

\item $h(N)=1\rightarrow$ my model with variable workload and $f(N)=1$, $g(N)=c_1 \cdot N^{\alpha}$
\item $h(N)=c_2 \cdot N^{\beta}t \rightarrow$ my model with variable workload and $f(N)=1$, $g(N)=c_1 \cdot N^{\alpha}$
\end{itemize}

\item Full model including (coordination and communication) overhead function: $T_1= f(N)\cdot s+g(N)\cdot p$; $T_N= f(N)\cdot s+\frac{g(N)\cdot p}{h(N)}+z(N)$
\begin{itemize}
\item concept of $T_0(N):=z(N)$ with some mathematical properties introduced by \citep{flatt1989performance}  
\end{itemize}

 
\end{itemize}

\section{Basic model}
\label{sec:basicModel}

This approach is a basic one and suggests a parameterized model which distinguishes Amdahl's law (strong scaling, problem size is constant) \cite{amdahl1967validity} and Gustafson's law (one type of weak scaling, problem size varies)\cite{gustafson1988reevaluating} along with different values of a single parameter $\alpha$. It is based on the following assumptions: 


\begin{itemize}
\item no coordination/communication overhead
\item overall amount of work involved in executing parallelizable part $p$ is invariant against serial or parallel execution
\item work/execution time of a single parallel processing unit = $s+pN^{\alpha}$ (Viewed from a more contemporary perspective, when models are relevant according to the workload realities of any particular scenario)
\end{itemize}


Note that
\begin{itemize}
	\item this model has been proposed by Sun and Ni as the memory-bounded speedup model \cite{sun1990another,sun1993scalable}
	\item $\alpha=0 \leftarrow$ Amdahl's law, $\alpha=1\leftarrow$ Gustafson's law (``scaled speedup''), $\alpha=0.5\leftarrow$ ``generalized scaled speedup" \cite{juurlink2012amdahl}
\end{itemize}


\begin{landscape}

$
{\def\arraystretch{1.3}\begin{array}{l|c|cc|c}
\alpha   & \mbox{work/serial time} & \multicolumn{2}{c|}{\mbox{parallel}}   & \mbox{speedup} \\
         &                         & \mbox{time}     & \mbox{performance}    & \\
\hline
\alpha=0~ \mbox{(Amdahl)} & s+p=1                    & s+\frac{p}{N}        & \frac{1}{s+\frac{p}{N}} & \frac{s+p}{s+\frac{p}{N}} \xrightarrow[N\to \infty]{} \frac{s+p}{s} = \frac{1}{s}  \qquad (\Theta(1))\\
\hline
\alpha=1~ \mbox{(Gustafson)} & s+pN                  & s+\frac{pN}{N}=s+p=1 & \frac{1}{s+p}=1  & \frac{s+pN}{s+p} = s+pN \xrightarrow[N\to \infty]{}\infty \qquad (\Theta(N)) \\
\hline
\mbox{general}               & s+pN^\alpha           & s+\frac{pN^\alpha}{N} = s+pN^{\alpha -1}  & \frac{1}{s+pN^{\alpha -1}} & \begin{array}{rl}
\frac{s+pN^{\alpha}}{s+pN^{\alpha -1}} & = \frac{s}{s+pN^{\alpha -1}} + \frac{pN^{\alpha}}{s+pN^{\alpha -1}} =  \frac{s}{s+pN^{\alpha -1}} + \frac{pN}{s{N^{1-\alpha}}+p}\\
                                       & \xrightarrow[N\to \infty]{\eqref{eq:first_term_basic},\eqref{eq:second_term_basic}}  
\left\{\begin{array}{cl}
0+\lim_{N\to \infty} N \qquad (\Theta(N))   & , \alpha > 1\\
s+\lim_{N\to \infty} pN \qquad (\Theta(N)) & , \alpha = 1\\
1+lim_{N\to \infty} \frac{pN^\alpha}{(1-\alpha)s} \qquad (\Theta(N^\alpha))                  & , 0 < \alpha < 1\\
1+\frac{p}{s}=\frac{s+p}{s}=\frac{1}{s} \qquad (\Theta (1))& , \alpha = 0\\
1+0=1 \qquad (\Theta (1))                 & , \alpha < 0
\end{array}\right. 
                                       
\end{array}
\end{array}}
$

\end{landscape}

%\vspace{1cm}

\begin{equation}
\lim_{N\to \infty} \frac{s}{s+pN^{\alpha -1}} =
\left\{\begin{array}{cl}
\frac{s}{s} = 1   & , \alpha < 1\\
\frac{s}{s+p} = s & , \alpha = 1\\
0                 & , \alpha > 1
\end{array}\right. \label{eq:first_term_basic}
\end{equation}

\vspace{1cm}


\begin{equation}
\lim_{N\to \infty}\frac{pN}{s{N^{1-\alpha}}+p} =
\left\{\begin{array}{cl}
\lim_{N\to \infty} \frac{p}{p}N = \lim_{N\to \infty} N   & , \alpha > 1\\
\lim_{N\to \infty} pN  & , \alpha = 1\\
\eqref{eq:lhospital} \lim_{N\to \infty} \frac{pN^\alpha}{(1-\alpha)s}                  & , 0 < \alpha < 1\\
\lim_{N\to \infty} \frac{p}{s}=\frac{p}{s} & , \alpha = 0\\
\eqref{eq:lhospital} \lim_{N\to \infty} \frac{pN^\alpha}{(1-\alpha)s}=0             & , \alpha < 0
\end{array}\right. \label{eq:second_term_basic}
\end{equation}

\vspace{1cm}

\begin{equation}
\lim_{N\to \infty} f(x) = \lim_{N\to \infty} g(x) = \infty \xRightarrow[]{\mbox{L'Hospital}} \lim_{N\to \infty} \frac{f(N)}{g(N)} = \lim_{N\to \infty} \frac{f'(N)}{g'(N)} \label{eq:lhospital}
\end{equation}

\textbf{Key findings: The results indicate that
\begin{itemize}
\item asymptotic speedup is constant (e.g., in Amdahl' law), linear (e.g., Gustafson's law), or sublinear,
\item superlinear speedup cannot be explained with this model.
\end{itemize}
}    

\section{Model with flexible effects of parallelization}
\label{sec:ModelFlexibleEffects}

This approach aims at considering some practical effects of computational parallelization; it generalizes the basic model in two regards: a) the work/serial time is generalized by adding a factor $c_1$; b) the effect of using $N$ parallel computation units on the time required to execute the parallelizable part is flexible and does not assume that the total work that is executed in parallel is constant over $N$. This flexibility allows accounting for different effects: (1) As \cite{hill2008amdahl} note, software is not just infinitely parallel and sequential. (2) Adopting this approach allows modeling that parallelization leads to an increase of execution time (e.g., due to coordination and communication effects) or that the total workload of executing parallel code is reduced (e.g., due to effects of the order in which workload is executed). However, the model does not include an explicit term for coordination and communication efforts; it rather contains a term that subsumes both coordination and communication efforts and time savings achieved through distributing the parallelizable workload on parallel computing units. (3) total workload to be executed in parallel may depend on the (non-deterministic) behavior of parallel program execution and may even be reduced (e.g., in a branch-and-bound context).

This model is based on the following assumptions:    

\begin{itemize}
\item  coordination/communication overhead is not modeled explicitly (but is covered to some extent when $\beta<1$)
\item overall amount of work involved in executing parallelizable part may vary (divided by $c_2N^{\beta}, c_2>0$) (e.g., in case of b\&b procedures this may occur when parallelization affects (parallel) workload because early pruning of subtrees makes solving some subtrees obsolete)\footnote{Kommentar Philipp: Das Phaenomen tritt meines Wissens sogar allgemeiner bei einigen "backtracking"-Verfahren auf (BaB als Spezialfall).}
\item work/execution time of a single parallel processing unit = $s+p\cdot(c_1N^{\alpha}),c_1>0$ (generalization of abovementioned used function)   
\end{itemize}


Note
\begin{itemize}
	\item  $c_1=c_2=1, \alpha=0, \beta=1 \leftarrow$ Amdahl's law
	\item  $c_1=c_2=1, \alpha=\beta=1\leftarrow$ Gustafson's law 
	\item  $c_1=c_2=1, \beta=1 \leftarrow$ speedup model of Sun and Ni ($\bar g (m)=m^b$ corresponds to $N^{\alpha}$) (The fundamental assumption leading to Sun–Ni's model is that the speedup is memory-bounded; However, with Sun–Ni's model, the size of
these larger problems would be limited by memory and not the number of cores (see paper)
	\item  $c_1=c_2=1, \alpha=0.5, \beta=1 \leftarrow$ speedup model of \cite{juurlink2012amdahl}
	\item This model is identical to the model in the previous section when $c_1=c_2=\beta$.
\end{itemize}


may be insert graphics such as those in \cite[Fig. 5]{juurlink2012amdahl}
Work/serial time: $ s+p\cdot(c_1 N^{\alpha}) $ \qquad Parallel time: $ s+\frac{p\cdot(c_1 N^{\alpha})}{c_2 N^{\beta}}=s+\frac{p\cdot c_1}{c_2}N^{\alpha - \beta} $ \qquad Parallel performance: $ \frac{1}{s+\frac{p\cdot c_1}{c_2}N^{\alpha - \beta}} $\\

Speedup: $ \frac{s+p\cdot (c_1 N^{\alpha})}{s+\frac{c_1p}{c_2}N^{\alpha - \beta}} = \underbrace{\frac{s}{s+\frac{c_1p}{c_2}N^{\alpha - \beta}}}_{(I)} + \underbrace{\frac{p\cdot (c_1 N^{\alpha})}{s+\frac{c_1p}{c_2}N^{\alpha - \beta}}}_{(II)}$\\
\vspace*{1cm}

ad (I):
\begin{equation}
 \lim_{N\to \infty} \frac{s}{s+\frac{c_1p}{c_2}N^{\alpha - \beta}}=
 \left\{\begin{array}{cl}
  0 & , \alpha > \beta\\
  \frac{s}{s+\frac{c_1p}{c_2}} & , \alpha = \beta\\
  1 & , \alpha < \beta\\
  \end{array}\\
 \right. \label{eq:first_term_varParWorkload} 
\end{equation} 

ad (II):\\

Case 1: $\alpha<0$ or $\beta<0$
\begin{equation}
 \lim_{N\to \infty} \frac{p\cdot (c_1 N^{\alpha})}{s+\frac{c_1 p}{c_2} N^{\alpha - \beta}}=\lim_{N\to \infty} \frac{p\cdot c_1}{sN^{-\alpha}+\frac{c_1 p}{c_2}N^{-\beta}}=0
 \label{eq:second_term_varParWorkload} 
\end{equation} 

Case 2: $\alpha=0$
\begin{equation}
\lim_{N\to \infty} \frac{p\cdot (c_1 N^{\alpha})}{s+\frac{c_1 p}{c_2} N^{\alpha - \beta}}=\lim_{N\to \infty} \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}N^{-\beta}}=
 \left\{\begin{array}{cl}
  \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}} & , \beta = 0 \\
  0 & , \beta < 0 \\
  \frac{p\cdot c_1}{s} & , \beta > 0\\
  \end{array}\\
 \right. \label{eq:third_term_varParWorkload} 
\end{equation}

Case 3: $\beta=0$
\begin{equation}
\lim_{N\to \infty} \frac{p\cdot (c_1 N^{\alpha})}{s+\frac{c_1 p}{c_2} N^{\alpha - \beta}}=\lim_{N\to \infty} \frac{p\cdot c_1}{sN^{-\alpha}+\frac{c_1 p}{c_2}}=
 \left\{\begin{array}{cl}
  \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}} & , \alpha = 0 \\
  0 & , \alpha < 0 \\
  \frac{p\cdot c_1}{\frac{p\cdot c_1}{c_2}}=c_2 & , \alpha > 0\\
  \end{array}\\
 \right. \label{eq:fourth_term_varParWorkload} 
\end{equation}

Case 4: $\alpha,\beta>0$
\begin{equation}
\lim_{N\to \infty} \frac{p\cdot (c_1 N^{\alpha})}{s+\frac{c_1 p}{c_2} N^{\alpha - \beta}}=
 \left\{\begin{array}{cl}
  \lim_{N\to \infty} \frac{p\cdot c_1}{s}N^{\alpha} & , \alpha < \beta \\
  \lim_{N\to \infty} \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}}N^{\alpha} & , \alpha = \beta \\
  \lim_{N\to \infty} \frac{p\cdot c_1 N^{\alpha-(\alpha-\beta)}}{\frac{s}{N^{\alpha-\beta}}+\frac{c_1 p}{c_2}} = \lim_{N\to \infty} \frac{p\cdot c_1 N^{\beta}}{\frac{s}{N^{\alpha-\beta}}+\frac{c_1 p}{c_2}} = \lim_{N\to \infty} \frac{p\cdot c_1 N^{\beta}}{\frac{p\cdot c_1}{c_2}}= \lim_{N\to \infty} c_2\cdot N^{\beta} & , \alpha > \beta \\
  \end{array}\\
 \right. \label{eq:fifth_term_varParWorkload} 
\end{equation}

Joining the limits of functions in (I) and (II) yields the limits of the speedup:

\begin{equation}
\lim_{N\to \infty} \frac{s+p\cdot (c_1 N^{\alpha})}{s+\frac{c_1p}{c_2}N^{\alpha - \beta}}=
 \left\{\begin{array}{lll}
 0+0=0 & (\Theta (1))&, \beta<\alpha<0\\[2mm]
 \frac{s}{s+\frac{c_1 p}{c_2}} + 0 = \frac{s}{s+\frac{c_1 p}{c_2}} & (\Theta (1))&, \beta=\alpha<0\\[2mm]
 1+0=1 & (\Theta (1))&, \beta>\alpha; \alpha<0\\[2mm]
 0+0=0 &(\Theta (1))&, \beta<\alpha; \beta<0\\[2mm]
 \frac{s}{s+\frac{c_1 p}{c_2}} + 0 = \frac{s}{s+\frac{c_1 p}{c_2}} &(\Theta (1))&, \alpha=\beta<0\\[2mm]
 1+0=1 &(\Theta (1))&, \alpha<\beta<0\\[2mm]
 \frac{s}{s+\frac{c_1 p}{c_2}} + \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}} = \frac{s+p\cdot c_1}{s+\frac{c_1 p}{c_2}} &(\Theta (1))&, \beta=\alpha=0\\[2mm]
 0+0=0 & (\Theta (1))&, \beta<\alpha=0\\[2mm]
 1+\frac{p\cdot c_1}{s} & (\Theta (1))&, \beta>\alpha=0\\[2mm]
 0+c_2=c_2 &(\Theta (1))&, \alpha>\beta=0\\[2mm]
 \frac{s}{s+\frac{c_1 p}{c_2}} + \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}} = \frac{s+p\cdot c_1}{s+\frac{c_1 p}{c_2}} &(\Theta (1))&, \alpha=\beta=0\\[2mm]
  1+0=1 &(\Theta (1))&, \alpha<\beta=0\\[2mm]
  \frac{s}{s+\frac{c_1 p}{c_2}} + \lim_{N\to \infty} \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}}N^{\alpha}=\lim_{N\to \infty} \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}}N^{\alpha} &(\Theta (N^{\alpha}))&, \alpha=\beta; \alpha,\beta>0\\[2mm]
  1 +  \lim_{N\to \infty} \frac{p\cdot c_1}{s}N^{\alpha}=\lim_{N\to \infty} \frac{p\cdot c_1}{s}N^{\alpha}&(\Theta (N^{\alpha}))&, \alpha<\beta; \alpha,\beta>0\\[2mm]
  0 +  \lim_{N\to \infty} c_2 N^{\beta}=\lim_{N\to \infty} c_2 N^{\beta}&(\Theta (N^{\beta}))&, \alpha>\beta; \alpha,\beta>0\\
  \end{array}\\
 \right. \label{eq:sixth_term_varParWorkload} 
\end{equation}

An alternative, matrix-based representation of these results is given in Table \ref{tab:results_varParWorkload}.

\begin{landscape}

\begin{table}[hb]
\center
\label{tab:results_varParWorkload}
\begin{tabular}{c|c|c|c|c|p{9cm}}
& & \multicolumn{3}{c|}{$\alpha$} & \multirow{2}{*}{\begin{minipage}{9cm}{Interpretation: The parallelizable part, when executed in parallel, requires computation times which $\ldots$} \end{minipage}}\\
\cline{3-5}
& & $<0$ & $=0$ & $>0$  & \\
\hline
\multirow{7}{*}{$\beta$}& \multirow{3}{*}{$<0$} & $0, \beta<\alpha$ & \multirow{3}{*}{$0$} & \multirow{3}{*}{$0$} & $\ldots$ increase with increasing $N$ (e.g., coordination and communication costs exceed parallelization savings)\\[2mm]
                        &                      & $\frac{s}{s+\frac{c_1 p}{c_2}}, \beta=\alpha$ &                      &                      & \\[2mm]
                        &                      & $1, \beta>\alpha$ &                      &                      &\\     
\cline{2-6}
                        & $=0$                 & $1$               & $\frac{s+p\cdot c_1}{s+\frac{c_1 p}{c_2}}$				    & $c_2$				  & $\ldots$ is constant (independent of $N$); i.e.; balance of a) coordination and coordination costs and b)parallelization savings)\\
\cline{2-6}
						& \multirow{3}{*}{$>0$}& \multirow{3}{*}{$1$} & \multirow{3}{*}{$1+\frac{p\cdot c_1}{s}$} & $\lim_{N\to \infty} c_2 N^{\beta}, \beta<\alpha$ &$\ldots$ decrease with increasing $N$ (due to parallelization savings)\\[2mm]
						&					  &                      &                                & $\lim_{N\to \infty} \frac{p\cdot c_1}{s+\frac{c_1 p}{c_2}}N^{\alpha},\beta=\alpha $ &\\[2mm]
						&					  &                      &                                & $ \lim_{N\to \infty} \frac{p\cdot c_1}{s}N^{\alpha},\beta>\alpha$ &\\	
						\hline		
\multicolumn{2}{l|}{\begin{minipage}{3cm}{Interpretation: Work/execution time of a single parallel unit $\ldots$} \end{minipage}} 			  & \begin{minipage}{3cm}{$\ldots$ decreases with increasing $N$: unreasonable in practice} \end{minipage} & \begin{minipage}{3cm}{$\ldots$ is constant and does not depend on $N$ (e.g., in Amdahl's law}) \end{minipage}& \begin{minipage}{3cm}{$\ldots$ increases with increasing $N$: (e.g., in Gustafons's law}) \end{minipage}&		    			                                                
\end{tabular} 
\caption{Summary of limits of speedup functions}
\end{table}

\end{landscape}

These results can be further summarized as follows: 
\begin{equation}
\text{speedup}=
 \left\{\begin{array}{ll}
 \Theta (N^{\alpha})&, \alpha\leq\beta;\alpha,\beta>0\\[2mm]
 \Theta (N^{\beta})&, \alpha>\beta;\alpha,\beta>0\\[2mm]
 \Theta (1) &, otherwise
   \end{array}   
 \right.
 =\left\{\begin{array}{ll}
 \Theta (N^{\min{(\alpha,\beta)}})&, \min{(\alpha,\beta)} > 0\\[2mm]
 \Theta (1) &, otherwise
   \end{array}
   \right.\\ \label{eq:seventh_term_varParWorkload} 
\end{equation}



\textbf{Key findings: The results indicate that asymptotic speedup is
\begin{itemize}
\item superlinear iff $\min\{\alpha,\beta\}>1$,  
\item linear iff $\min\{\alpha,\beta\}=1$,
\item sublinear iff $0<\min\{\alpha,\beta\}<1$,
\item constant iff $\min\{\alpha,\beta\}\leq 0$  
\end{itemize}
}    

Comment on modeling coordination and communication cost: Although the model allows considering these costs with $\beta<0$, the term $N^{\beta}$, which subsumes both the aforementioned costs and time savings through parallelization, is either strictly monotonically increasing or strictly monotone decreasing. However, in practical computations, the aggregation of both effects often leads to overall time savings before, at a break-even point $N^{\ast}$, the time required for executing the parallel workload starts increasing as coordination costs exceed parallelization time savings. Thus, it deems practically useful to add a term to the execution time dedicated to coordination and communication costs.   

Our previous comment is in line with the statement of \cite{al2020amdahl}: Although it may be argued that the p-fraction may be viewed as capable of including the effects of non-processing activities such as communication and memory access to some extent, the quantitative relationship is far from straightforward. A single number parameter such as f may become semantically too weak to properly represent the complex effects of communications between different parts of a workload and accessing memory, which may require synchronisation and waiting in shared memory architectures such as most modern off-the-shelf processors.

Non-processing activities, referred to as ``overheads": coordination, communication, sysnchronization (Synchronisation overheads are the effects on the performance of the joining and handshaking of multiple processes and data), memory-wall (characterizes the effects of the memory-processor performance gap on the entire system.)

\section{Model with overheads}

"cost of synchronization/overheads"; the tradeoff between parallelism and granularity \cite{flatt1989performance}; reasons for costs: critical regions (exclusive access for one process only), inter-process communication, and sequential-to-parallel synchronization (due to data exchange) \citep{yavits2014effect}; Generally, communication overheads cause large performance degradation in multi-core collaboration \cite{huang2013extending}   

compared to the model suggested in the previous section, this model provides three extensions: a) effects of increasing number of parallel processing units on serial fraction $s$ (why?); b) flexible functions for two effects on parallelization part; b) extends cost function $z$ for overhead through parallelization (coordination etc.)

remark wrt. overhead function $z$:
\begin{itemize}
  \item may be considered a penalty term
  \item additive overheads of all types have been covered in the literature, e.g.,
  \begin{itemize}
  \item overhead of data preparation \citep{pei2016extending}
  \item   communication time (The communication time is the time required for the inter-core communication necessitated by mapping a workload onto multiple cores.) considered in the extension of Amdahl's law in \cite{li1988analysis}, which i summarized in \cite[p. 137]{al2020amdahl}
  \item further work refernned in \cite[p. 137]{al2020amdahl}: Chen, X., Lu, Z., Jantsch, A., et al.: ‘Speedup analysis of data-parallel applications on multi-core NoCs’. IEEE 8th Int. Conf. on ASIC, Changsha,
People's Republic of China, October 2009, pp. 105–108; 
\end{itemize}
\item   add a coefficient function to the parallel part of the denominator of Amdahl's law; e.g., Eyerman, S., Eeckhout, L.: ‘Modeling critical sections in Amdahl's law and its implications for multicore design’, SIGARCH Comput. Archit. News, 2010,
38, (3), pp. 362–370. Available at http://doi.acm.org/; Sun, X.H., Ni, L.M.: ‘Another view on parallel speedup’. Proc. Super
Computing ‘90, New York NY, USA, November 1990, pp. 324–333 10.1145/1816038.1816011 

  
   \item theoretical model: \cite{flatt1989performance}, see below
\end{itemize}

Work/serial time: $ f(N)\cdot s + p\cdot g(N) $ \qquad Parallel time: $ f(N) \cdot s+\frac{g(N) \cdot p}{h(N)}+z(n) $ \qquad Parallel performance: $ \frac{1}{f(N) \cdot s+\frac{g(N) \cdot p}{h(N)}+h(z)} $\\

Speedup: $ \frac{f(N)\cdot s + p\cdot g(N)}{f(N) \cdot s+\frac{g(N) \cdot p}{h(N)}+z(n)}$\\


comment on $g(N)$: our term $p \cdot g(N)$ is in line with \cite{juurlink2012amdahl}: In this equation the amount of work that can be parallelized
is not constant as in Amdahl's law, nor does it grow linearly with the number of cores as in Gustafson's law. Instead, the
amount of parallel work is proportional to a function scale(p) that is sub-linear in p (e.g., scale(p) = $\sqrt{N}$p


functions do not reflect asymmetric environments: to consider those, they would probably need to inlcude some more parameters which describe the heterogeneity  

\subsection{Model of Flatt and Kennedy}

\cite{flatt1989performance}:
\begin{itemize}
\item key assumption (Amdahl's assumption of a sequential and a parallelizable part + an overhead function): $T(n)=T_s+\frac{T_P}{n}+T_0(n)$
\item The impact of synchronization and communication overhead on the performance of parallel processors
is investigated to establish upper bounds on the performance of parallel processors under ideal
conditions. Bounds are derived under fairly general conditions on the synchronization cost function.

\item share the assumption of Amdahl' law: for a given program, there is a region amenable to parallel execution and this region can be partitioned
into as many tasks of equal duration as we like.

\item analyzing the behavior of reasonable choices for the overhead function $T_o(n)$. This function represents the contribution to running time due to the need for synchronization and communication between processors. Its value can be affected by the structure of the application, which influences the necessity for communication, the task dispatching algorithm used to control the assignment of processes to processors, and the hardware and software mechanisms for communication and synchronization.

\item some mathematical assumptions on the overhead function $T_o(n)$ (linear and log. functions included) lead to the fact that there is a unique number $n_0$ of parallel processing units at which the the overall execution time gets the global minimum value; i.e., values of $n$ below or above $n_0$ lead to longer execution times! (theorem 3.4)
\item performance measure:
\begin{itemize}
\item parallel cost penalty: $Q(n)=nT(n)=\frac{nT(n}{1\cdot (T(1)}$ is the ratio of the cost of renting $n$ processing units for time period $T(n)$ (cost of parallel execution) to the cost of renting $1$ processor for $1$ unit of time (cost of serial execution); parallel cost penalty $Q(n)$ and $Q'(n)$ are both monotone increasing
\item efficiency: $E(n)=\frac{1}/{Q(n)}$; efficiency $E(n)$ is monotone increasing, $E'(n)$ is monotone increasing
\item Speedup: $S(n)=\frac{1}{T(n)}=n\cdot E(n)=\frac{n}{Q(n)}$: the speedup $S(n)$ has a unique maximum at $n_0>=1$ (We note that this is a stronger result than Amdahl's Law [2,5], which predicts a maximum speedup of $\frac{1}{T_s}$ that cannot be achieved with a finite number of processors. The principal difference here is the effect of the overhead function $T_0(n)$.)
\item operating point: From the previous discussion, it is clear that neither the efficiency nor the speedup alone gives a good indicator of where the best operating point should be. The best efficiency is achieved with one processor, while efficiency will be less than $1/2$ for a machine with $n_0$ processors. We should be able to pick some number of processors $< n_0$ for which the efficiency is much greater but the speedup is not significantly smaller. We need to somehow take both efficiency and speedup into consideration when picking such a point: speedup over cost:$F(n)=\frac{S(n}{n\cdot T(n)}S(n) \cdot E(n)$; there exists a unique value of $n$, say $n_F$, at which $F(n)$ assumes a maximum for $n\geq 1$; $n_F$ is the optimal point for $\frac{S(n)}{\sqrt(n)}$; $S'(n_F)=\frac{S(n_f)}{2n_F}<\frac{1}{2}$
\end{itemize} 
\item new assumption/setting to define scaled speedup for varying workloads: 
\begin{itemize}
	\item we will define the running time T to be a function of both the number of processors n and a measure z of the number of elementary computations in a given algorithm: $T(n,z)=T_s(z)+\frac{T_p(z)}{n}+T_0(n,z)$
	\item Scaled speedup $S(k,n,z)=k\cdot \frac{T(n,z)}{T(kn,kz}$; $n \geq $ is the original number of processors and $z > 0$ is the
original number of computations
	\item Note: this def. of scaled speedup is inconsistent with Gustafson's definition because: setting $n=1$ and ignoring coordination cost function $T_0(n,k)$ results to a ratio $\frac{k\cdot T(1,z)}{T(k,kz)}=\frac{k\cdot (T_s(z)+T_p(z))}{T(k,kz)}=\frac{k\cdot (T_s+T_p)}{T_s+T_p}\neq \frac{T_s+T_p\cdot k}{T_s+T_p} $ (if $T_s\neq 0$ and $k\neq 1$)
	\item under some specific scalability assumptions, scaled speedup is upper-bounded by O(1) ! (in contrast to Gustafson's law): however; Gustafson ignores communication overhead
\end{itemize}
\end{itemize}


\section{Related work}

\subsection{General commments on parallelization}

Prominent models suggested in the literature \citep{sun2010reevaluating,rafiev2018speedup}:
\begin{itemize}
\item Amdahl's law: fixed-size speedup model 
\item Gustafson's law: fixed-time speedup model 
\item Sun and Ni's law: memory-bounded speedup model (generalization of Amdahl's law and of Gustafson's law): Since many algorithms have a polynomial complexity in terms of computation and memory requirement, and we can always take the highest degree term to represent the complexity of the algorithm \cite{sun1990another,sun1993scalable}

\end{itemize}


Amdahl's law has been criticized for several reasons. To assess these issues, it is important to identify and evaluate the assumptions implicitly made in this law: (1) problem size is fixed,(2) no overhead induced through communication, synchronization, etc. is considered. As a result, the computed speedup and its upper bound are too high from a practical perspective. (3) Performance improvements (in particular, in serial and parallel regions) are presumed to be isolated from one another; or, more precisely, resources upon which the regions execute are both unbounded and homogeneous. However, when resources must be viewed as a trade-off within a bounded (finite) space, this assumption no longer holds. \cite{paul2007amdahl}. Such effects are demonstrated by \cite{hill2008amdahl} who (mathematically) show that Amdahl's law, albeit valid, needs to be applied under varying conditions (symmetric, asymmetric, or dynamic multicore chips) and different resulting mathematical instantiations of Amdahl's law.  

Gustafson's law: scale of the workload is in the parallel processing part only


\subsection{Heterogenous processing units}

The initial assumption of all models covered and developed in this paper, parallel processing units are equally potential in their computing capabilities, is not always given. In this subsection, we biefly outline approaches to cover effiiciency when the assumption is violated; i.e., not all parallel processing units have the identical processing capabilities.

overview of Amdahl's law (and othe rlaws) for heterogenous MCP is given by \cite{al2020amdahl}; a prior Survey on Amdahl's Law Extension in Multicore Architectures is provided by \citep{al2013survey} 

This section is not a review in that it does not provide a comprehensive list of references.

an overview of literature on architectures and performance effects of HeMCP system (incorporates a number of different cores that may have different architecture) is provided by \citep[p. 139]{al2020amdahl}.

application of laws to multi-core chips:
\begin{itemize}
	\item studies on architecture-dependent laws are particularly helpful for the design of multi-core chips

	\item recent review of Amdahl's law in the context of heterogeneous many-core systems \cite{al2020amdahl}
 
    \item effects of various designs of multicore chips on parallel speedup based on Amdahl \cite{hill2008amdahl}
    
    \item We apply Gustafson's law to symmetric, asymmetric, and dynamic multicores \cite{juurlink2012amdahl}
    
    \item we propose speedup models for manycore architecture in this paper. Under the assumption of Hill-Marty model, we deduce our formulas based on Gustafson’s Law and Sun-Ni’s Law \cite{Ye2013}
    
    \item \citet{rafiev2018speedup} generalize the laws of Amdahl and Gustafson; they suggest a normal-form model which that supports a wide range of heterogeneous many-core architectures and which defines the system’s parallel performance via the performance-equivalent number of BCEs (‘base core equivalent’), which [BCE) may be understood as a basic core capable of performing the workload in question with a performance of 1 (unit performance).; their generalization of Amdahl's law leads to a generalization of Hill and Marty's model   
    
    \item \citep{zidenberg2012multiamdahl}: We introduce MultiAmdahl, an analytical optimization technique for resource sharing among heterogeneous units, journal version: \citep{zidenberg2013optimal}; \citep{morad2012generalized} extend this model to a generalized MultiAmdahl model
    
    \item \citep{moncrieff1996heterogeneous}: We consider the implications of Amdahl’s Law for a heterogeneous system of computers each of which is a homogeneous parallel processor. We introduce a parallelism profile function to describe the level of parallelism achieved in different fragments of the computation
    \begin{itemize}
    \item assumptions: heterogeneous two-node system (extendable to n machines) with each node having SMC arhitectures, i.e., cores on the two machines have different and fixed peak rates (similar to Hill and Marty who provde in their dynamic model for th eoption to combine several BCEs to one processing unit with increased computing capability (e.g., in term sof peak performance)); algorithm may have several fragments each of which shows different levels of parallelism (in contrast to Amdahl and Hill and Marty, who foresees just one level of parallelism), fragments are executed sequentially on either of the 2 machines; overall, this model generalizes the Hill and Marty model logically (albeit technologically targeting a different architecture) 
    \item authors analyze the speedup when each fragment is assigned to that machine which executes the fragment most efficiently  
    \end{itemize}     
\end{itemize}
 
extension of laws to multi-core chips; the extensions consider overheads:

\begin{itemize}
	\item \cite{yavits2014effect}: 
	\begin{itemize}
		\item considers overhead; based on the model of \cite{hill2008amdahl} as a reference framework
		\item A modification of Amdahl’s law is formulated, to reflect the finding that parallel speedup is lower than originally predicted, due to these effects; Parallelization incurs data exchange between the sequential core and the parallel cores at the beginning and the end of each parallel section of a program (sequential-to-parallel synchronization), and the data exchange among the parallel cores during parallel execution (inter-core communication). This paper investigates the effect of these synchronization and communication elements on multicore performance, speedup, and scaling.

		\item Our novel multicore performance model accounts for the effects of a) data synchronization and b) inter-core communication: a) In between parallel and sequential segments, data are synchronized, namely transferred between the two memories, as indicated by the double arrows in the two figures. That transfer is named sequential to parallel synchronization; b) During parallel execution, the multiple cores may exchange data. That inter-core communication comprises the second limiting effect studied in this paper; the inter-core connectivity time and connectivity intensity strongly depend on the specifics of each workload as well as the actual implementation of the architecture, for example, the number of cores.

	\end{itemize}


\item \cite{huang2013extending}: extension of of Amdahl's law and Gustafson's law (in architecture-sepcific multi-core settings) by considering communication overheads and area constraints

\item \cite{eyerman2010modeling}: Modeling Critical Sections in Amdahl’s Law and its Implications for Multicore Design

\item \cite{pei2016extending}: Overheads from such actions as memory access, on-chip communications and synchronisation among cores: Extending Amdahl's law for heterogeneous multicore processor with consideration of the overhead of data preparation 

\item \cite{morad2006performance}: The interactions between multiple parallel processors incur performance overheads. These overheads are a result of synchronization, communication and coherence costs; based upon Amdahl's model

\end{itemize}
\begin{figure}
\includegraphics[width=\linewidth]{overviewModels.jpg}
\caption{Overview of speedup models}
\end{figure}
offene Punkte

\begin{itemize}
\item noch lesen: https://www.goodreads.com/book/show/1085126.Introduction\_to\_Parallel\_Computing
\item Trennung von alg. und techn. Aspekten (memory wall z.B.) möglich, oder sollte auch mein Modell memory wall issues aufgreifen? 
\end{itemize}


